Equilibria and Learning in Modular Marketplaces

We envision a marketplace where diverse entities offer specialized "modules" through APIs, allowing users to compose the outputs of these modules for complex tasks within a given budget. This paper studies the market design problem in such an ecosystem, where module owners strategically set prices for their APIs (to maximize their profit) and a central platform orchestrates the aggregation of module outputs at query-time. One can also think about this as a first-price procurement auction with budgets. The first observation is that if the platform's algorithm is to find the optimal set of modules then this could result in a poor outcome, in the sense that there are price equilibria which provide arbitrarily low value for the user. We show that under a suitable version of the "bang-per-buck" algorithm for the knapsack problem, an $\varepsilon$-approximate equilibrium always exists, for any arbitrary $\varepsilon > 0$. Further, our first main result shows that with this algorithm any such equilibrium provides a constant approximation to the optimal value that the buyer could get under various constraints including (i) a budget constraint and (ii) a budget and a matroid constraint. Finally, we demonstrate that these efficient equilibria can be learned through decentralized price adjustments by module owners using no-regret learning algorithms.

==> tikz/additive_iterations.tex <==

\newcommand{\plotAdditiveIterationOne}[1]{
\begin{tikzpicture}[scale=#1]
  \begin{axis}[
    xlabel={$v$ (value)},
    ylabel={$p$ (price)},
    title={Budget 9, iteration 1},
    xmin=0, xmax=6,
    ymin=0, ymax=6,
    axis x line*=bottom,
    axis y line*=left,
  ]
    \acceptedCoords{
      (5, 1) 
    };

    \rejectedCoords{
      (2, 1)
      (3, 3)
      (1, 4)
    };

    \node[above] at (axis cs:5,1) {$1$};
    \node[below] at (axis cs:5,1) {$(5, 1)$};

    \node[above] at (axis cs:2,1) {$2$};
    \node[below] at (axis cs:2,1) {$(2, 1)$};

    \node[above] at (axis cs:3,3) {$3$};
    \node[below] at (axis cs:3,3) {$(3, 3)$};

    \node[above] at (axis cs:1,4) {$4$};
    \node[below] at (axis cs:1,4) {$(1, 4)$};

    \addplot[dashed, domain=0:6] {x / 5};
  \end{axis}
\end{tikzpicture}
}

\newcommand{\plotAdditiveIterationTwo}[1]{
\begin{tikzpicture}[scale=#1]
  \begin{axis}[
    xlabel={$v$ (value)},
    ylabel={$p$ (price)},
    title={Budget 9, iteration 2},
    xmin=0, xmax=6,
    ymin=0, ymax=6,
    axis x line*=bottom,
    axis y line*=left,
  ]
    \acceptedCoords{
      (5, 2.5) 
      (2, 1)
    };

    \rejectedCoords{
      (3, 3)
      (1, 4)
    };

    \node[above] at (axis cs:5,2.5) {$1$};
    \node[below] at (axis cs:5,2.5) {$(5, 2.5)$};

    \node[above] at (axis cs:2,1) {$2$};
    \node[below] at (axis cs:2,1) {$(2, 1)$};

    \node[above] at (axis cs:3,3) {$3$};
    \node[below] at (axis cs:3,3) {$(3, 3)$};

    \node[above] at (axis cs:1,4) {$4$};
    \node[below] at (axis cs:1,4) {$(1, 4)$};

    \addplot[dashed, domain=0:6] {x / 2};
  \end{axis}
\end{tikzpicture}
}

\newcommand{\plotAdditiveIterationThree}[1]{
\begin{tikzpicture}[scale=#1]
  \begin{axis}[
    xlabel={$v$ (value)},
    ylabel={$p$ (price)},
    title={Budget 9, iteration 3},
    xmin=0, xmax=6,
    ymin=0, ymax=6,
    axis x line*=bottom,
    axis y line*=left,
  ]
    \acceptedCoords{
      (5, 4.75) 
      (2, 1.9)
    };

    \rejectedCoords{
      (3, 3)
      (1, 4)
    };

    \node[above] at (axis cs:5,4.75) {$1$};
    \node[below] at (axis cs:5,4.75) {$(5, 5(1-\delta))$};

    \node[above] at (axis cs:2,1.9) {$2$};
    \node[below] at (axis cs:2,1.9) {$(2, 2(1-\delta))$};

    \node[above] at (axis cs:3,3) {$3$};
    \node[below] at (axis cs:3,3) {$(3, 3)$};

    \node[above] at (axis cs:1,4) {$4$};
    \node[below] at (axis cs:1,4) {$(1, 4)$};

    \addplot[dashed, domain=0:6] {0.95 * x};
  \end{axis}
\end{tikzpicture}
}

\newcommand{\plotAdditiveIterationBOne}[1]{
\begin{tikzpicture}[scale=#1]
  \begin{axis}[
    xlabel={$v$ (value)},
    ylabel={$p$ (price)},
    title={Budget 5.25, iteration 1},
    xmin=0, xmax=6,
    ymin=0, ymax=6,
    axis x line*=bottom,
    axis y line*=left,
  ]
    \acceptedCoords{
      (5, 1) 
    };

    \rejectedCoords{
      (2, 1)
      (3, 3)
      (1, 4)
    };

    \node[above] at (axis cs:5,1) {$1$};
    \node[below] at (axis cs:5,1) {$(5, 1)$};

    \node[above] at (axis cs:2,1) {$2$};
    \node[below] at (axis cs:2,1) {$(2, 1)$};

    \node[above] at (axis cs:3,3) {$3$};
    \node[below] at (axis cs:3,3) {$(3, 3)$};

    \node[above] at (axis cs:1,4) {$4$};
    \node[below] at (axis cs:1,4) {$(1, 4)$};

    \addplot[dashed, domain=0:6] {x / 5};
  \end{axis}
\end{tikzpicture}
}

\newcommand{\plotAdditiveIterationBTwo}[1]{
\begin{tikzpicture}[scale=#1]
  \begin{axis}[
    xlabel={$v$ (value)},
    ylabel={$p$ (price)},
    title={Budget 5.25, iteration 2},
    xmin=0, xmax=6,
    ymin=0, ymax=6,
    axis x line*=bottom,
    axis y line*=left,
  ]
    \acceptedCoords{
      (5, 2.5) 
      (2, 1)
    };

    \rejectedCoords{
      (3, 3)
      (1, 4)
    };

    \node[above] at (axis cs:5,2.5) {$1$};
    \node[below] at (axis cs:5,2.5) {$(5, 2.5)$};

    \node[above] at (axis cs:2,1) {$2$};
    \node[below] at (axis cs:2,1) {$(2, 1)$};

    \node[above] at (axis cs:3,3) {$3$};
    \node[below] at (axis cs:3,3) {$(3, 3)$};

    \node[above] at (axis cs:1,4) {$4$};
    \node[below] at (axis cs:1,4) {$(1, 4)$};

    \addplot[dashed, domain=0:6] {x / 2};
  \end{axis}
\end{tikzpicture}
}

\newcommand{\plotAdditiveIterationBThree}[1]{
\begin{tikzpicture}[scale=#1]
  \begin{axis}[
    xlabel={$v$ (value)},
    ylabel={$p$ (price)},
    title={Budget 5.25, iteration 3},
    xmin=0, xmax=6,
    ymin=0, ymax=6,
    axis x line*=bottom,
    axis y line*=left,
  ]
    \acceptedCoords{
      (5, 3.75) 
      (2, 1.5)
    };

    \rejectedCoords{
      (3, 3)
      (1, 4)
    };

    \node[above] at (axis cs:5,3.75) {$1$};
    \node[below] at (axis cs:5,3.75) {$(5, 3.75)$};

    \node[above] at (axis cs:2,1.5) {$2$};
    \node[below] at (axis cs:2,1.5) {$(2, 1.5)$};

    \node[above] at (axis cs:3,3) {$3$};
    \node[below] at (axis cs:3,3) {$(3, 3)$};

    \node[above] at (axis cs:1,4) {$4$};
    \node[below] at (axis cs:1,4) {$(1, 4)$};

    \addplot[dashed, domain=0:6] {0.75 * x};
  \end{axis}
\end{tikzpicture}
}
